Hardware-efficient autonomous quantum error correction

We propose a new method to autonomously correct for errors of a logical qubit induced by energy relaxation. This scheme encodes the logical qubit as a multi-component superposition of coherent states in a harmonic oscillator, more specifically a cavity mode. The sequences of encoding, decoding and correction operations employ the non-linearity provided by a single physical qubit coupled to the cavity. We layout in detail how to implement these operations in a practical system. This proposal directly addresses the task of building a hardware-efficient and technically realizable quantum memory.

==> qubitreset.tex <==
\Qcircuit @C=2em @R=1.5em {
\lstick{\begin{array}{l}c_g \ket{\alpha'(1\minou i)}\\ \plusou c_e e^{i\tfrac{\pi}{4}}e^{i{\bar n'}}\ket{0} \end{array}}&
\qw&
\qw&
\rstick{\begin{array}{l}c_g \ket{\alpha'(1\minou i)}\\ \plusou c_e e^{i\tfrac{\pi}{4}}e^{i{\bar n'}}\ket{0} \end{array}}
\\
\lstick{\tfrac{e^{-2i{\bar n'}}\ket{g}\pm\ket{e}}{\sqrt{2}}}&
\gate{\text{Reset}}&
\qw&
\rstick{\ket{g}}
}
